WOUAF: Weight Modulation for User Attribution and Fingerprinting in Text-to-Image Diffusion Models

The rapid advancement of generative models, facilitating the creation of hyper-realistic images from textual descriptions, has concurrently escalated critical societal concerns such as misinformation. Although providing some mitigation, traditional fingerprinting mechanisms fall short in attributing responsibility for the malicious use of synthetic images. This paper introduces a novel approach to model fingerprinting that assigns responsibility for the generated images, thereby serving as a potential countermeasure to model misuse. Our method modifies generative models based on each user's unique digital fingerprint, imprinting a unique identifier onto the resultant content that can be traced back to the user. This approach, incorporating fine-tuning into Text-to-Image (T2I) tasks using the Stable Diffusion Model, demonstrates near-perfect attribution accuracy with a minimal impact on output quality. Through extensive evaluation, we show that our method outperforms baseline methods with an average improvement of 11\% in handling image post-processes. Our method presents a promising and novel avenue for accountable model distribution and responsible use. Our code is available in \url{https://github.com/kylemin/WOUAF}.

==> sec/X_suppl_bak.tex <==
\clearpage
%\setcounter{page}{1}
\maketitlesupplementary
\appendix

\section{Additional Related Work}
\label{app:related_work}
\paragraph{Text-to-Image Generative Models}
Recent advancements in vector quantization and diffusion modeling have significantly enhanced text-to-image (T2I) generation, enabling the creation of hyper-realistic images from textual prompts~\citep{nichol2022glide,saharia2022photorealistic,ramesh2022hierarchical, stable_diffusion}. These T2I models have been effectively utilized in various tasks such as generating images driven by subject, segmentation, and depth cues~\cite{chefer2023attend, chen2023training, patel2023conceptbed, patel2024lambda,gal2022image, li2023gligen}. However, the substantial size of these models presents a challenge for broader user adoption. Research efforts are focusing on enhancing model efficiency through knowledge distillation, step distillation, architectural optimization, and refining text-to-image priors~\cite{li2023snapfusion, salimans2021progressive, luo2023latent,patel2023eclipse}. Amidst these technological advancements, ensuring the responsible usage of these powerful tools is a critical area of focus, which is the aim of our proposed method.


\paragraph{Image Watermarking}
Image watermarking aims to embed a watermark into images for asserting copyright ownership. To maintain the original image's fidelity, these watermarks are embedded imperceptibly. Traditional approaches often employ Fourier or Wavelet transforms, while recent advancements leverage deep neural network-based auto-encoders for this purpose~\cite{rivagan,zhu2018hidden,tancik2020stegastamp}. However, as discussed in the main paper, these methods can be easily disabled in an open-source setting.

From the standpoint of ownership verification, the fingerprinting of generative models aligns conceptually with watermarking techniques. However, unlike direct image manipulation to embed an identifiable signal in watermarking, generative model fingerprinting embeds this signal within the model's weights. Consequently, the identifiable signal is integrated during the image generation process, akin to leaving fingerprints. This approach inherently prevents users from dissociating the fingerprinting process from image generation.


\paragraph{Neural Network Watermarking}
Watermarking techniques, particularly those embedding unique identifiers within model parameters, have been substantively explored in various studies, such as those highlighted in~\cite{adi2018turning, ong2021protecting, uchida2017embedding, darvish2019deepsigns, wang2021riga}. Our methodology, while aligning with the foundational principles of these works, introduces notable advancements in several key areas: utility, scalability, and verification methodology. The majority of existing watermarking techniques are tailored towards image classification models, with only a limited subset extending their applicability to generative models, each presenting its own set of limitations. Unlike traditional methods that predominantly target single classification models, our approach endeavors to fingerprint approximately 4 billion Text-to-Image generator instances through a singular fine-tuning process. Additionally, while prior works have embedded fingerprints into various model aspects, such as input-output dynamics~\cite{adi2018turning, ong2021protecting} or directly within model weights~\cite{uchida2017embedding, darvish2019deepsigns,wang2021riga}, our strategy diverges by eliminating the necessity for trigger input, thereby enhancing scalability. In the context of our problem domain, where malicious users rarely share their model weights with the distributor responsible for watermark verification, the distributor typically only has access to potentially misused images. In essence, our approach not only aligns with but also extends beyond the conventional boundaries of network watermarking techniques, ensuring a thorough inclusion and discussion of these foundational methods in our related works section.


\section{Additional Details}
WOUAF is evaluated utilizing the Stable Diffusion (SD) model~\cite{stable_diffusion} (version 2-base), trained specifically for generating images of 512p resolution.

\section{Additional Experimental Results}
%Section explanation
In addition to the figure in the main paper, we added uncurated images using text-prompt from MS-COCO~\cite{lin2014microsoft} and LAION Aesthetics~\cite{schuhmann2022laion}.
For convenience, we have aligned the subsection names with those in the main manuscript. Unless otherwise specified, all figures were generated using the `WOUAF-all' method.

\subsection{Additional Training Details}
The dimension of the mapping network $d_M$ is set to be equal to $4*d_\phi$ across all experimental setups. Training is performed over 50K iterations with a batch size of 32 and a learning rate of $10^{-4}$ using AdamW optimizer~\cite{adamw}. 

\subsection{Attribution Accuracy and Image Quality}
% 4.3 -> uncurated image collection (5 each)

As highlighted in the main manuscript, our methodology has a negligible effect on the original Stable Diffusion's image quality. Please refer to Fig.~\ref{fig:supp_uncurated} for these uncurated images.

\begin{figure*}[h]
\centering
  \includegraphics[width=\textwidth]{images/supp_uncurated.pdf} \\ \hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Uncurated images of the original and fingerprinted Stable Diffusion models on MS-COCO and LAION Aesthetics. Pixel-wise differences are multiplied by a factor of 5 for a better view.}
  \label{fig:supp_uncurated}
\end{figure*}


\subsection{Evaluating Generalizability Across Datasets} % imagenet training model -> Figure 4.. (5)


\begin{figure*}[!htbp]
\centering
  \includegraphics[width=\textwidth]{images/supp_imagenet.pdf} \\ \hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Qualitative comparisons of the original and fingerprinted Stable Diffusion models that were fine-tuned using only the ImageNet dataset. Pixel-wise differences are multiplied by a factor of 5 for a better view.}
  \label{fig:supp_imagenet}
\end{figure*}

\begin{table*}[!htbp]
\centering
\caption{Assessment of attribution accuracy and generation quality using Imagenet trained models. We validated our method using MS-COCO testset and LAION-aesthetics dataset. $\uparrow$/$\downarrow$ indicates higher/lower is desired.}
\label{tab:attribution_imagenet}
{\small
\begin{tabularx}{\textwidth}{lXXXXXX}
\toprule
\multirow{3}{*}{Model} & \multicolumn{3}{c}{MS-COCO} & \multicolumn{3}{c}{LAION} \\
 & Attribution Acc. ($\uparrow$) & Clip-score ($\uparrow$)& FID ($\downarrow$)& Attribution Acc. ($\uparrow$) & Clip-score ($\uparrow$)& FID ($\downarrow$)\\
\midrule
Ours-conv. & 0.99 & 0.73 & 24.23 & 0.99 & 0.51 & 19.71 \\
Ours-all & 0.99 & 0.73 & 24.41 & 0.99 & 0.51 & 19.46 \\
\bottomrule
\end{tabularx}
}
\vspace{-0.1in}
\end{table*}


A key feature of our proposed methodology is its design independence from image-text paired datasets for achieving attribution accuracy. This property imbues it with the potential for broad applicability across a diverse range of contexts. To substantiate this claim, we conducted an experiment in which our variant models were trained exclusively on the ImageNet dataset~\cite{deng2009imagenet}.
We subsequently evaluated the performance of these ImageNet-trained models on the MS-COCO test set as well as a randomly selected portion of the LAION-aesthetics datasets. 

The evaluation results, as seen in Table~\ref{tab:attribution_imagenet}, effectively corroborate our assertion. Our methodology demonstrates compelling performance, with both our variants, achieving high attribution accuracy and maintaining image generation quality. These results underscore our method's independence from the use of text-image paired datasets, thereby establishing its broad applicability in diverse scenarios where reliable fingerprinting and high-quality image generation are required. Fig.~\ref{fig:supp_imagenet} provides a visual representation of these images.





\subsection{Attribution Accuracy Across Various Generation Hyperparameters}
% robustness -> similar to table 1, Figures


\begin{table*}[t]
\centering
\caption{Assessment of attribution accuracy and generation quality using Euler and DDIM scheduler with different time steps on MS-COCO. We fixed classifier-free guidance scale~\cite{ho2022classifier} to \textbf{7.5}.
$\uparrow$/$\downarrow$ indicates higher/lower is desired.}
\label{tab:hyperparam_1}
{\small
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
\toprule
\multirow{3}{*}{Model} & \multicolumn{4}{c}{Euler~\cite{euler}} & \multicolumn{4}{c}{DDIM~\cite{ddim}} \\\cmidrule(lr){2-5} \cmidrule(lr){6-9}
  & Steps & Attribution Acc. ($\uparrow$)  & CLIP-score ($\uparrow$)& FID ($\downarrow$) & Steps & Attribution Acc. ($\uparrow$) & CLIP-score ($\uparrow$)& FID ($\downarrow$)\\
\midrule
Original SD~\cite{stable_diffusion} & 20 & - & 0.73 & 24.48 & 50 & - & 0.73 & 23.33 \\
\midrule
%De
\multirow{3}{*}{WOUAF-conv} & 15 & 0.99 & 0.73 & 24.63 & 45 & 0.99 & 0.73 & 23.28 \\
 & 20 & 0.99 & 0.73 & 24.43 & 50 & 0.99 & 0.73 & 23.35 \\
 & 25 & 0.99 & 0.74 & 24.14 & 55 & 0.99 & 0.73 & 23.31 \\
%qkvde
\midrule
\multirow{3}{*}{WOUAF-all} & 15 & 0.99 & 0.73 & 24.65 & 45 & 0.99 & 0.73 & 23.34 \\
 & 20 & 0.99 & 0.73 & 24.42 & 50 & 0.99 & 0.73 & 23.29 \\
 & 25 & 0.99 & 0.73 & 24.11 & 55 & 0.99 & 0.73 & 23.26 \\
\bottomrule
\end{tabularx}
}
\vspace{-0.1in}
\end{table*}


\begin{table*}[t]
\centering
\caption{Assessment of attribution accuracy and generation quality on different classifier-free guidance scales~\cite{ho2022classifier} using MS-COCO. We fixed the scheduler and time steps to Euler for \textbf{20} steps and DDIM for \textbf{50} steps.
$\uparrow$/$\downarrow$ indicates higher/lower is desired.}
\label{tab:hyperparam_2}
{\small
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
\toprule
\multirow{3}{*}{Model} & \multicolumn{4}{c}{Guidance Scale 2.5} & \multicolumn{4}{c}{Guidance Scale 5.0} \\\cmidrule(lr){2-5} \cmidrule(lr){6-9}
  & Scheduler & Attribution Acc. ($\uparrow$)  & CLIP-score ($\uparrow$)& FID ($\downarrow$) & Scheduler & Attribution Acc. ($\uparrow$) & CLIP-score ($\uparrow$)& FID ($\downarrow$)\\
\midrule
%De
\multirow{2}{*}{WOUAF-conv} & Euler & 0.99 & 0.72 & 18.63 & Euler & 0.99 & 0.73 & 21.91 \\
 & DDIM & 0.99 & 0.72 & 18.35 & DDIM & 0.99 & 0.73 & 20.78 \\
%qkvde
\midrule
\multirow{2}{*}{WOUAF-all} & Euler & 0.99 & 0.71 & 18.64 & Euler & 0.99 & 0.73 & 21.89 \\
 & DDIM & 0.99 & 0.71 & 18.31 & DDIM & 0.99 & 0.73 & 20.68 \\
\bottomrule
\end{tabularx}
}
\vspace{-0.1in}
\end{table*}


\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{images/various_1.pdf}
  \caption{Qualitative results obtained using the Euler and DDIM schedulers with varying time steps on the MS-COCO dataset. We maintained a constant classifier-free guidance scale~\cite{ho2022classifier} at \textbf{7.5}. Each column corresponds to the 'WOUAF-all' rows in Table~\ref{tab:hyperparam_1}.}
  \label{fig:supp_various_1}
\end{figure*}

\begin{figure*}[t]
\centering
  \includegraphics[width=0.88\textwidth]{images/various_2.pdf}
  \caption{Qualitative results produced by applying different classifier-free guidance scales~\cite{ho2022classifier} on the MS-COCO dataset. The scheduler and time steps were held constant at Euler for \textbf{20} steps and DDIM for \textbf{50} steps. Each column aligns with the 'WOUAF-all' rows in Table~\ref{tab:hyperparam_2}.}
  \label{fig:supp_various_2}
\end{figure*}



In accordance with the details provided in the primary manuscript, we subjected our methodology to evaluation employing two widely accepted schedulers: Euler~\cite{euler}, featuring time steps at intervals of [15, 20, 25], and DDIM~\cite{ddim}, operating at time steps in [45, 50, 55]. Along with these, we also incorporated classifier-free guidance scales~\cite{ho2022classifier} at 2.5, 5.0, and 7.5.

Echoing the discussions in the main paper, the data in Tab.~\ref{tab:hyperparam_1} and~\ref{tab:hyperparam_2} corroborate the near-perfect attribution accuracy achieved by our method. Furthermore, the absence of significant deterioration in quality metrics reaffirms the resilience of our approach in the face of diverse generation hyperparameters (Refer to Fig.~\ref{fig:supp_various_1} and Fig.~\ref{fig:supp_various_2}).





\subsection{Benefits of Finetuning only Decoder}

In this section, we present qualitative outcomes resulting from the joint fine-tuning of the Stable Diffusion model's components, diffusion model $\epsilon_\theta$ and decoder $\mathcal{D}$. 
As accentuated in the primary manuscript, our training protocol achieved an accuracy of 89\%, however, it resulted in a noticeable deterioration in the quality metrics (Clip-score: 0.68, FID: 63.48).
Fig.~\ref{fig:supp_unet_decoder} provides additional visual affirmation of these quantitative results.



\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{images/supp_unet.pdf} \\ \hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Qualitative results of the original and fingerprinted Stable Diffusion models on MS-COCO and LAION Aesthetics. When fine-tuning the SD model's $\epsilon_\theta$ and $\mathcal{D}$ together, there are significant quality drops. Pixel-wise differences are multiplied by a factor of 5 for a better view.}
  \label{fig:supp_unet_decoder}
\end{figure*}


\subsection{Robust User Attribution against Image Post-processes}
%Quality table de, qkvde together

\begin{figure*}
\centering
  \includegraphics[width=\textwidth]{images/atk_sample.pdf} \\ %\hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Examples of images after applying each of the post-processing methods that we consider in the paper.}
  \label{fig:atk_samples}
\end{figure*}

We conducted a thorough evaluation of quality metrics to assess the impact of our robust user attribution training on various image post-processing methods. Examples of images post-processed using these methods are displayed in~\cref{fig:atk_samples}. As indicated in~\cref{tab:robust_fid} and~\cref{tab:robust_clip}, our robust fine-tuning approach generally preserves image quality with only minimal perturbations. A representative example under a JPEG attack, generated by our robust model, is showcased in Fig.~\ref{fig:supp_post_jpeg}.
Additionally, our method demonstrates adaptability under Combination attacks, which significantly challenge image fidelity. As illustrated in~\cref{fig:atk_samples}, these combined post-processing techniques necessitate a relatively stronger fingerprint compared to single post-processes, as further detailed in~\cref{fig:supp_post_all}.


\begin{table*}[t]
\centering
\caption{FID~\cite{heusel2017gans} scores using MS-COCO after robust training. 
Lower is desired.}
\label{tab:robust_fid}
{\small
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
\toprule
Model & Crop & Rotation & Blur& Brightness& Noise & Erasing & JPEG& Combi.\\
\midrule
%De
WOUAF-conv & \multirow{2}{*}{24.02} & \multirow{2}{*}{24.05} & \multirow{2}{*}{23.80} & \multirow{2}{*}{24.14} & \multirow{2}{*}{23.96} & \multirow{2}{*}{24.16} & \multirow{2}{*}{24.42} & \multirow{2}{*}{26.80} \\
(robust) &  &  &  &  &  &  &  &  \\
%qkvde
WOUAF-all & \multirow{2}{*}{24.35} & \multirow{2}{*}{23.92} & \multirow{2}{*}{24.18} & \multirow{2}{*}{24.54} & \multirow{2}{*}{24.24} & \multirow{2}{*}{24.48} & \multirow{2}{*}{24.41} & \multirow{2}{*}{26.85} \\
(robust) &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabularx}
}
\vspace{-0.1in}
\end{table*}

\begin{table*}[t]
\centering
\caption{CLIP scores~\cite{hessel2021clipscore} using MS-COCO after robust training. 
Higher is desired.}
\label{tab:robust_clip}
{\small
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
\toprule
Model & Crop & Rotation & Blur& Brightness& Noise & Erasing & JPEG& Combi.\\
\midrule
%De
WOUAF-conv & \multirow{2}{*}{0.716} & \multirow{2}{*}{0.717} & \multirow{2}{*}{0.716} & \multirow{2}{*}{0.716} & \multirow{2}{*}{0.712} & \multirow{2}{*}{0.717} & \multirow{2}{*}{0.714} & \multirow{2}{*}{0.702} \\
(robust) &  &  &  &  &  &  &  &  \\
%qkvde
WOUAF-all & \multirow{2}{*}{0.719} & \multirow{2}{*}{0.717} & \multirow{2}{*}{0.718} & \multirow{2}{*}{0.718} & \multirow{2}{*}{0.710} & \multirow{2}{*}{0.718} & \multirow{2}{*}{0.716} & \multirow{2}{*}{0.704} \\
(robust) &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabularx}
}
\vspace{-0.1in}
\end{table*}



\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{images/supp_post_jpeg.pdf} \\ \hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Qualitative results of the original and fingerprinted Stable Diffusion models on MS-COCO and LAION aesthetics. Our fingerprinted model is trained by simulating JPEG compression during training. Pixel-wise differences are multiplied by a factor of 5 for a better view.}
  \label{fig:supp_post_jpeg}
\end{figure*}


\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{images/supp_post_all.pdf} \\ \hspace*{6.5em}(a) MS COCO \hspace{12.5em}(b) LAION Aesthetics
  \caption{Qualitative results of the original and fingerprinted Stable Diffusion models on MS-COCO and LAION aesthetics. Our fingerprinted model is trained by simulating all the combinations of the post-processing during training. Pixel-wise differences are multiplied by a factor of 5 for a better view.}
  \label{fig:supp_post_all}
\end{figure*}

\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{images/gaussian_atk.pdf}
  \caption{Model Purification. Adding Gaussian noise into weights leads to concurrent declines in both image quality and attribution accuracy. Note that a lower FID score is preferable, indicating better image quality.}
  \label{fig:gaussian_atk}
\end{figure}

\section{Additional Deliberate Fingerprint Manipulation}
\subsection{Gaussian Noise Model Purification}
This subsection addresses the scenario where an adversary, upon recognizing the presence of fingerprints within the images generated by the image decoder $\mathcal{D}$, opts to add Gaussian noise into $\mathcal{D}$ to obliterate the embedded fingerprint. In order to test this scenario, we gradually increase the standard deviation following $[0., 0.01, 0.015, 0.02, 0.025, 0.03]$. As shown in~\cref{fig:gaussian_atk}, our empirical analysis reveals a significant challenge: efforts to decrease the attribution accuracy lead to a decline in the quality of the generated images. This result also supports the idea that efforts to decrease attribution accuracy lead to a significant decline in the quality of the generated images.


\subsection{Full Knowledge Attack Scenario}
This scenario assumes an internal attacker with comprehensive knowledge of our training process, including the training dataset, model structure, fingerprint space, and training details. To validate this, we trained an attacker's version, following our methodology but employing a different random seed. We then assessed user attribution accuracy by inputting 5K images generated by the attacker's model into WOUAF-conv and WOUAF-all fingerprint decoding networks. Both of our model variants exhibited user attribution accuracies of \textbf{0.509} and \textbf{0.501}, which are essentially random guesses, and thus dodged the attack. Even when an attacker with complete knowledge replicates our methodology, they will not be able to mislead the original fingerprint decoding network.
